PSM: Learning Probabilistic Embeddings for Multi-scale Zero-Shot Soundscape Mapping

A soundscape is defined by the acoustic environment a person perceives at a location. In this work, we propose a framework for mapping soundscapes across the Earth. Since soundscapes involve sound distributions that span varying spatial scales, we represent locations with multi-scale satellite imagery and learn a joint representation among this imagery, audio, and text. To capture the inherent uncertainty in the soundscape of a location, we design the representation space to be probabilistic. We also fuse ubiquitous metadata (including geolocation, time, and data source) to enable learning of spatially and temporally dynamic representations of soundscapes. We demonstrate the utility of our framework by creating large-scale soundscape maps integrating both audio and text with temporal control. To facilitate future research on this task, we also introduce a large-scale dataset, GeoSound, containing over $300k$ geotagged audio samples paired with both low- and high-resolution satellite imagery. We demonstrate that our method outperforms the existing state-of-the-art on both GeoSound and the existing SoundingEarth dataset. Our dataset and code is available at https://github.com/mvrl/PSM.

==> sec/table.tex <==
\begin{table*}[ht!]
\centering
\begin{tabular}{@{}lccccccc@{}}
\toprule
method & metadata type                              & inference meta & \multicolumn{1}{c|}{zoom level} & I2S R@10 & I2S median rank & S2I R@10 & S2I median rank \\ \midrule
\multicolumn{8}{c}{bingmap}                                                                                        \\ \midrule
baseline~\citep{khanal2023soundscape} & none                                        & 0 & \multicolumn{1}{c|}{1} & 0.4012 & 1507 & 0.4042 & 1468 \\ \midrule
ours  & none                                        & 0 & \multicolumn{1}{c|}{1} & 0.4215 & 1389 & 0.4263 & 1339 \\
ours  & withmeta      & 1 & \multicolumn{1}{c|}{1} & 0.4255 & 1359 & 0.4452 & 1241 \\
ours  & withmeta      & 0 & \multicolumn{1}{c|}{1} & 0.8263 & 261  & 0.8294 & 247  \\
ours  & withmeta+text & 0 & \multicolumn{1}{c|}{1} & 0.9015 & 113  & 0.9432 & 100  \\ \midrule
baseline~\citep{khanal2023soundscape} & none                                        & 0 & \multicolumn{1}{c|}{3} & 0.4090 & 1438 & 0.4198 & 1382 \\ \midrule
ours  & none                                        & 0 & \multicolumn{1}{c|}{3} & 0.4410 & 1307 & 0.4413 & 1260 \\
ours  & withmeta      & 1 & \multicolumn{1}{c|}{3} & 0.4365 & 1315 & 0.4521 & 1215 \\
ours  & withmeta      & 0 & \multicolumn{1}{c|}{3} & 0.8260 & 268  & 0.8313 & 253  \\
ours  & withmeta+text & 0 & \multicolumn{1}{c|}{3} & 0.9013 & 113  & 0.9449 & 101  \\ \midrule
baseline~\citep{khanal2023soundscape} & none                                        & 0 & \multicolumn{1}{c|}{5} & 0.4107 & 1427 & 0.4206 & 1371 \\ \midrule
ours  & none                                        & 0 & \multicolumn{1}{c|}{5} & 0.4409 & 1308 & 0.4469 & 1267 \\
ours  & withmeta      & 1 & \multicolumn{1}{c|}{5} & 0.4239 & 1386 & 0.4422 & 1246 \\
ours  & withmeta      & 0 & \multicolumn{1}{c|}{5} & 0.8211 & 277  & 0.8251 & 263  \\
ours  & withmeta+text & 0 & \multicolumn{1}{c|}{5} & 0.8966 & 117  & 0.9391 & 107  \\ \midrule
\multicolumn{8}{c}{sentinel}                                                                                       \\ \midrule
baseline~\citep{khanal2023soundscape} & none                                        & 0 & \multicolumn{1}{c|}{1} & 0.4585 & 1183 & 0.4657 & 1147 \\ \midrule
ours  & none                                        & 0 & \multicolumn{1}{c|}{1} & 0.4738 & 1107 & 0.4849 & 1056 \\
ours  & withmeta      & 1 & \multicolumn{1}{c|}{1} & 0.4647 & 1145 & 0.4770 & 1099 \\
ours  & withmeta      & 0 & \multicolumn{1}{c|}{1} & 0.8030 & 296  & 0.8073 & 285  \\
ours  & withmeta+text & 0 & \multicolumn{1}{c|}{1} & 0.8724 & 142  & 0.9402 & 104  \\ \midrule
baseline~\citep{khanal2023soundscape} & none                                        & 0 & \multicolumn{1}{c|}{3} & 0.4525 & 1204 & 0.4570 & 1189 \\ \midrule
ours  & none                                        & 0 & \multicolumn{1}{c|}{3} & 0.4760 & 1090 & 0.4897 & 1034 \\
ours  & withmeta      & 1 & \multicolumn{1}{c|}{3} & 0.4735 & 1116 & 0.4945 & 1014 \\
ours  & withmeta      & 0 & \multicolumn{1}{c|}{3} & 0.7977 & 309  & 0.8018 & 292  \\
ours     & withmeta+text & 0              & \multicolumn{1}{c|}{3}                 & 0.8696    & 151         & 0.9403    & 104.5       \\ \midrule
baseline~\citep{khanal2023soundscape} & none                                        & 0 & \multicolumn{1}{c|}{5} & 0.4583 & 1196 & 0.4563 & 1186 \\ \midrule
ours  & none                                        & 0 & \multicolumn{1}{c|}{5} & 0.4582 & 1163 & 0.4664 & 1141 \\
ours  & withmeta      & 1 & \multicolumn{1}{c|}{5} & 0.4695 & 1119 & 0.4903 & 1034 \\
ours  & withmeta      & 0 & \multicolumn{1}{c|}{5} & 0.7966 & 314  & 0.7977 & 300  \\
ours  & withmeta+text & 0 & \multicolumn{1}{c|}{5} & 0.8679 & 155  & 0.9365 & 109  \\ \bottomrule
\end{tabular}
\caption{Main experiment table }
\label{tab:main_retrieval}
\end{table*}
